Age Minimization with Energy and Distortion Constraints

In this paper, we consider a status update system, where an access point collects measurements from multiple sensors that monitor a common physical process, fuses them, and transmits the aggregated sample to the destination over an erasure channel. Under a typical information fusion scheme, the distortion of the fused sample is inversely proportional to the number of measurements received. Our goal is to minimize the long-term average age while satisfying the average energy and general age-based distortion requirements. Specifically, we focus on the setting in which the distortion requirement is stricter when the age of the update is older. We show that the optimal policy is a mixture of two stationary, deterministic, threshold-based policies, each of which is optimal for a parameterized problem that aims to minimize the weighted sum of the age and energy under the distortion constraint. We then derive analytically the associated optimal average age-cost function and characterize its performance in the large threshold regime, the results of which shed critical insights on the tradeoff among age, energy, and the distortion of the samples. We have also developed a closed-form solution for the special case when the distortion requirement is independent of the age, arguably the most important setting for practical applications.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> conclusion.tex <==
\section{Conclusion}
\ifreport
In this chapter, 
\else
In this paper, 
\fi 
we investigate an age minimization problem with constraints on the long-term average energy consumption and distortion of each update. The problem is formulated as a constrained MDP. Through the Lagrangian multiplier technique, we connect the problem to an average cost problem \eqref{avg_cost}, and show that the optimal policy is a mixture of two stationary deterministic policies (Theorem \ref{Ori_Lag}), each of which is optimal for the average cost problem and of a threshold-type (Theorem \ref{opt_stru}). Then, we obtain the average cost under the threshold-type policy, which is a piecewise function of threshold (Theorem \ref{cost_cal}), and we find the optimal threshold value in the last interval (Theorem \ref{new}). With these, we avoid dealing with infinite state space when using a classical solution RVI, and develop low-complexity algorithms. In the special case of the average cost problem, we obtain a closed-form solution (Corollary \ref{cor: special_case}). We show that the optimal threshold increases with the probability that distortion requirement is met, and the impact of transmission error probability $p$ on the optimal threshold depends on whether it is age or energy being the dominant issue (Theorem \ref{lem:special_case}).



% conference papers do not normally have an appendix


% use section* for acknowledgment
%\section*{Acknowledgment}


%The authors would like to thank...





% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)



==> model.tex <==
\section{system model}
\label{scheduler}
We consider a status update system, in which an access point collects samples from multiple sensors, combines the samples to form update and then transmits the update to a remote monitor/receiver, as shown in Fig. \ref{sysmodel}.
We consider a time-slotted system and we use $t\in\{1,2,\cdots\}$ to index each time slot. At the beginning of each time slot, $M$ sensors sample the same physical process from their own view and attempt to transmit samples to the access point over the wireless channels. Then, the access point decides whether to transmit an update, which consists of all collected samples, to the remote monitor, i.e., selecting action $u_{t} \in \mathcal{U}\triangleq\{0,1\}$, where $u_{t}=1$ means transmission, and $u_{t}=0$ denotes suspension of the transmission.

We assume that all channels are error-prone. Specifically, the error probability of a transmission from the sensor $m$ to the access point is $q_m$, for $m\in\{1,2,\cdots,M\}$, and the error probability of the transmission from the access point to the receiver is $p$. 
\ifreport
\begin{figure}[h]
    \centering
    \includegraphics[width=0.65\textwidth]{Age_dist/SysModel.pdf}
    \caption{System Model}
    \label{sysmodel}
\end{figure}
\else 
\begin{figure}[h]
\vspace{-0.2cm}
    \centering
    \includegraphics[width=0.36\textwidth]{SysModel.pdf}
    \caption{System Model}
    \vspace{-0.5cm}
    \label{sysmodel}
\end{figure}
\fi




\subsection{Age of Information}
Age of information (AoI), or the age reflects the timeliness of the information at the receiver. It is defined as the time elapsed since the generation of the most recently received update at the receiver. Let $\Delta_{t}$ denote the age at the beginning of the time slot $t$. Let $U(t)$ denote the generation time of the last successfully received status update for time slot $t$. Then, $\Delta_{t}$ is given by $\Delta_{t}\triangleq t-U(t)$.

If the transmission of an update is not successful in a time slot, then the age increases by one, otherwise, the age drops to one. 
Then, the value of $\Delta_{t+1}$ is updated as follows:

\begin{align}
\label{age_update}
& \Delta_{t+1}=
 %\left\{
  \begin{cases}%{l l}  
  1 & \text{if transmission is successful}, \\  
  1+\Delta_{t} & \text{otherwise}. 
  \end{cases} %\right.		
\end{align}
We assume that $\Delta_1=1$.
\subsection{Distortion and Energy constraints}
\label{sec: const}
Since transmissions from sensors to the access point are not reliable, the number of samples collected by the access point at each time slot varies from $0$ to $M$.
Assume that the distortion of an update, which consists of all collected samples, depends on the number of collected samples. 
We use $\Lambda_t$ to denote the number of collected samples at time slot $t$. To guarantee the quality of each update, we suspend access-point transmission whenever $\Lambda_t<D(\Delta_t)$, where $D(\cdot)$ is a function that maps the age to the minimum number of samples required for transmission.

We assume that $D(\cdot)$ is a non-decreasing function of the age on $[1,\infty)$ (since the smallest age is 1). Since $\Lambda_t$ is of integer value, without loss of generality, $D(\cdot)$ can be viewed as a piecewise constant function, which consists of $L\in \mathbb{N}^+$ intervals. Let $\delta_l$ denote the leftmost point of the $l$-th interval for $ 1\leq l\leq L$ and $\delta_{L+1}=\infty$. Then, the $l$-th interval is $[\delta_l,\delta_{l+1})$ and $\delta_1=1$. We use $h_l$ to denote the value over the $l$-th interval of domain, i.e, $h_l=D(\delta_l)$. Given $1\leq l<l'\leq L$, we have $h_l<h_{l'}$.
We assume that $h_1\geq 1$ and $h_L\leq M$. This is reasonable since if $h_L> M$, the transmission will never be conducted after the age exceeds $\delta_L$.
Fig. \ref{fig:distfun_inc} provides an example of the distortion function, where $L=3$ and $M=8$.
\ifreport
\begin{figure}
    \centering
    \includegraphics[width=0.55\textwidth]{Age_dist/Dfun_inc.pdf}
    \caption{Example of distortion function}
    \label{fig:distfun_inc}
\end{figure}
\else
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{Dfun_inc.pdf}
    \caption{Example of distortion function}
    \vspace{-0.8cm}
    \label{fig:distfun_inc}
\end{figure}
\fi 
%We define the inverse function $D^{-1}(\cdot)$ as
%\begin{align}
%    D^{-1}(\Lambda)\triangleq \sup\{\Delta\in\mathbb{N}^+:D(\Delta)\leq\Lambda\}.
%\end{align}

%We assume that $D(\cdot)$ is a non-increasing function of the age (This assumption was also considered in \cite{bastopcu2021age}). This is based on the observation that if the age is high, scheduler may want to receive update faster, in which case the scheduler trades quality for fresh data and lowers its distortion requirement. 

%Let $J$ denote the smallest number of packets such that transmission is possible as the age exceeds some threshold, i.e. $J\triangleq \min \{m\in\mathbb{N}^+:\; \exists \Delta_0,\; \text{s.t.} \; m\geq D(\Delta), \forall \Delta\geq \Delta_0\}$. We assume $J\leq M$.
%This is reasonable, otherwise, the system never transmits any updates. We define the inverse function $D^{-1}(\cdot)$ on domain $\{J,J+1,\cdots\}$ as
%\begin{align}
  %  D^{-1}(\Lambda)\triangleq \min\{\Delta\in\mathbb{N}^+:D(\Delta)\leq\Lambda\}, \forall \Lambda\geq J.
%\end{align}
%Fig. \ref{distfun} provides an example of the distortion function. In the example, $J=2$. Whenever the access point collects less than 2 samples, update will not be sent.
%\begin{figure}[h]
  %  \centering
  %  \includegraphics[width=0.25\textwidth]{Dfun.pdf}
   % \caption{An example of $D(\cdot)$}
   % \label{distfun}
%\end{figure}


%Moreover, since sensors are usually powered by battery and thus energy limited, transmission should be scheduled appropriately to prolong sensors' life.
The access point consumes energy for each transmission. We assume that each transmission consumes the same energy which is normalized as one unit energy, a setting similar to \cite{tsai2021jointly}. To avoid excessive energy consumption, we employ a long-term average energy consumption constraint for the access point. Note that in the system, sensors take samples periodically, and their energy consumption is fixed and thus not included in our optimization problem.

%Note that if there is no energy constraint at the access point, then transmitting updates whenever the distortion requirement is satisfied is optimal. This is because suspending the transmission does not contribute to decreasing the age. However, repeated transmission attempts could result in excessive energy consumption, and could be impractical for sensors or IoT devices that are usually energy constrained. Accordingly, we employ a long-term average energy consumption constraint for the access point.


\subsection{Optimization Problem}
A transmission control policy $\pi=\{d_1,d_2,\cdots\}$ specifies the decision rules for each time slot, where a decision rule $d_t$ is a function that maps the past actions, past and current age and the number of collected samples to actions. 
Our objective is to design a transmission control policy $\pi$ that minimizes the following long-term average age

\begin{align}
	&\bar{A}(\pi)\triangleq \lim_{T \rightarrow \infty} \frac{1}{T}\mathbb{E_\pi}\big[\sum_{t=1}^T \Delta_t\big],
	\label{avg_age}
\end{align}
while the long-term average energy consumption $\bar{E}(\pi)$ must not exceed $E_{\text{max}}\in (0,1]$, i.e.
\begin{align}
	&\bar{E}(\pi)\triangleq \lim_{T \rightarrow \infty} \frac{1}{T}\mathbb{E_\pi}\big[\sum_{t=1}^T u_t\big]\leq E_\text{max},
	\label{avg_energy}
\end{align}
and the distortion requirement is satisfied, i.e.
\begin{align}
    \Lambda_t\geq u_t D(\Delta_t),\ \  \forall t\geq 1,\label{dist_req}
\end{align}
where $\mathbb{E}_\pi$ denotes expectation under policy $\pi$.



==> optimization_prob.tex <==
\section{Constrained MDP Formulation and Lagrangian Relaxation}
\label{sec: formulation}
\subsection{Constrained MDP Formulation}
\label{components}
The optimization problem can be formulated as a constrained MDP. The components of the MDP are as follows:

\textbf{States:} The system state consists of the age and the number of collected samples, i.e., the system state at time slot $t$ is denoted by a tuple $\mathbf{s}_t=(\Delta_t,\Lambda_t)$. Then, the state space is given by $\mathcal{S}\triangleq \{(\Delta,\Lambda): \Delta\in \mathbb{N}^+,  \Lambda\in\{0,1,\cdots,M\}\}$, which is infinite. 

\textbf{Actions:} Action set is $\mathcal{U}=\{0,1\}$ as defined in Section \ref{scheduler}. Due to distortion requirement in \eqref{dist_req}, $u=1$ can be taken only when $\Lambda\geq D(\Delta)$. Define $A_{\mathbf{s}_t}\triangleq \{u_t\in \mathcal{U}: \Lambda_t\geq u_t D(\Delta_t)\}$ as the admissible action set in state $\mathbf{s}_t$ which satisfies the distortion requirement. %For example, for state $\mathbf{s}_t=(D^{-1}(M),M)$, the admissible action set is $\{0,1\}$, while for state $\mathbf{s}_t=(D^{-1}(M),0)$, the admissible action set is $\{0\}$.
%For example, for any $m\in[1,M], s_t=(D^{-1}(m), m)$, the admissible action set is \{0,1\} while for state $s_t=(D^{-1}(m)+1, m)$, the admissible action set is $\{0\}$. 
For example, with distortion requirement in Fig. \ref{fig:distfun_inc}, we have $A_{(5, 5)}=\{0,1\}$ while $A_{(51, 5)}=\{0\}$. 

\textbf{Transition Probability:} Given the current state $\mathbf{s}_{t}= (\Delta_{t}, \Lambda_{t})$ and action $u_{t}$ at time slot $t$, the transition probability to the state $\mathbf{s}_{t+1}=(\Delta_{t+1}, \Lambda_{t+1})$ at the next time slot $t+1$, which is denoted by $P_{\mathbf{s}_{t}\mathbf{s}_{t+1}}(u_t)$, is defined as
 \begin{align}
	P_{\mathbf{s}_{t}\mathbf{s}_{t+1}}(u_t)&\triangleq\mathbb{P}(\mathbf{s}_{t+1}|\mathbf{s}_{t},u_{t})\notag\\
&=\mathbb{P}(\Delta_{t+1}|\Delta_t,u_t)P_\Lambda(\Lambda_{t+1})
\end{align}
where
\begin{align}
&\mathbb{P}(\Delta_{t+1}|\Delta_t,u_t)=
  \begin{cases}%{l l}  
  p & \text{if}\, \, u_{t}=1,\Delta_{t+1}=1+\Delta_t \\
  1-p & \text{if} \, \, u_{t}=1,\Delta_{t+1}=1,\\  
  1 &\text{if} \, \, u_{t}=0,\Delta_{t+1}=1+\Delta_t,\\
  0 & \text{otherwise},
  \end{cases}
\end{align}
and $P_\Lambda(\Lambda_{t+1})\triangleq\mathbb{P}(\Lambda\!=\!\Lambda_{t+1})$.
%\begin{equation}
 %   P_\Lambda(\Lambda_{t+1})\triangleq\mathbb{P}(\Lambda\!=\!\Lambda_{t+1})=\frac{(1-q)^{\Lambda_{t+1}}q^{M-\Lambda_{t+1}}\cdot M!}{\Lambda_{t+1}!(M-\Lambda_{t+1})!}
%\end{equation}

\textbf{Costs:} Given a state $\mathbf{s}_t=(\Delta_{t}, \Lambda_{t})$ and an action choice $u_t$ at time slot $t$, the cost of one slot is the age at the beginning of this slot, i.e., we have
\begin{equation}
	C_\Delta(\mathbf{s}_t,u_{t})=\Delta_{t}.
\end{equation}
Moreover, the energy consumption of one slot is
\begin{equation}
	C_E(\mathbf{s}_t,u_{t})=u_t.
\end{equation}

Let $\Pi$ denote the set of \emph{feasible} policies that satisfy the distortion constraint, i.e., $u_t\in A_{\mathbf{s}_t}$, $\forall t$. Then, the transmission control problem can be formulated as a constrained Average-age MDP: 

\textit{Problem 1 (Average-age MDP):}
\begin{alignat}{2}
\label{ori_prob}
 \bar{A}^\star\triangleq   \min_{\pi\in\Pi} \quad & \bar{A}(\pi)= \limsup_{T \rightarrow \infty} \frac{1}{T}\mathbb{E_\pi}\big[\sum_{t=1}^T C_\Delta(\mathbf{s}_{t},u_{t})\big] &  \\
    \mathrm{s.t.} \quad & \bar{E}(\pi)=\limsup_{T \rightarrow \infty} \frac{1}{T}\mathbb{E_\pi}\big[\sum_{t=1}^T C_E(\mathbf{s}_{t},u_{t})\big] \leq E_{\text{max}}, &   \nonumber
   % &\Lambda_t\geq u_t D(\Delta_t) . \nonumber 
\end{alignat}
where $\bar{A}^\star$ is the optimal average age.
\subsection{Lagrange Relaxation of the Constrained MDP}
To obtain the optimal transmission control policy, we reformulate the average-age MDP in \eqref{ori_prob} as a parameterized average cost MDP. Given Lagrange multiplier $\beta$, the instantaneous Lagrangian cost at time slot $t$ is defined by
\begin{align}
	C(\mathbf{s}_{t},u_{t};\beta)=C_\Delta(\mathbf{s}_{t},u_{t})+\beta C_E(\mathbf{s}_{t},u_{t}).
	\label{inst_lag_cost}
\end{align}
Then, the long-term average Lagrangian cost under policy $\pi$ is given by
\begin{align}
	&\bar{L}(\pi;\beta)= \lim_{T \rightarrow \infty} \frac{1}{T}\mathbb{E_\pi}\big[\sum_{t=1}^T C(\mathbf{s}_{t},u_{t}; \beta)\big].\label{Lag_main}
\end{align}

Then, we have an average cost MDP, which aims at obtaining a feasible optimal policy $\pi\in\Pi$ that minimizes the long-term average Lagrangian cost above:

\textit{Problem 2 (Average cost MDP):}
\begin{align}
	\bar{L}^\star(\beta)  \triangleq &\min_{\pi\in \Pi}  \bar{L}(\pi;\beta).
%	&\mathrm{s.t.} \quad  \Lambda_t\geq u_t D(\Delta_t) .
	\label{avg_cost}
\end{align}
where $\bar{L}^\star(\beta)$ is the optimal average Lagrangian cost with regard to $\beta$. %A policy is said to be \emph{average cost optimal} if it minimizes the average Lagrangian cost while satisfying the distortion requirement.

A policy is \emph{stationary} if the decision rule is independent of time, i.e., $d_{t}=d$, for all $t$. Moreover, a policy is \emph{randomized} if $d_t: \mathcal{S}\rightarrow \mathcal{P}(\mathcal{U})$ specifies a probability distribution on the set of actions. The policy is \emph{deterministic} if $d_t: \mathcal{S} \rightarrow \mathcal{U}$ chooses an action with certainty. 

\begin{theorem}
\label{Ori_Lag}
There exists a stationary randomized policy that solves the average-age MDP \eqref{ori_prob}. This policy can be expressed as a mixture of two stationary deterministic policies $\pi_{\beta^\star,1}$ and $\pi_{\beta^\star,2}$, where $\pi_{\beta^\star,1}$ and $\pi_{\beta^\star,2}$ differ in
at most a single state $\mathbf{s}$, and are both optimal policies for the average cost MDP \eqref{avg_cost} given $\beta^\star$. The mixture policy $\pi_{\beta^\star}$ uses $\pi_{\beta^\star,1}$ with probability $\mu$ and $\pi_{\beta^\star,2}$ with probability $1-\mu$ in state $s$; it uses either policy (since they coincide) in other states, where $\mu\in [0,1]$
\end{theorem}
\begin{proof-sketch}
Please see Appendix \ref{proof_ori_lag}.
\end{proof-sketch}
\vspace{0.1cm}
%\begin{proof}
%Please see Appendix \ref{proof_ori_lag}.
%\end{proof}

\section{Average Cost MDP with Non-decreasing Distortion Function}
\label{sec: average_cost}
In this section, we investigate optimal policies that solve \eqref{avg_cost}. In particular, we derive the structure of the optimal policies. With this, we obtain the expression of the average Lagrangian cost as a function of a threshold $k$ and prove a property of the function, which are used in designing low-complexity algorithms in Section \ref{sec:alg_design}. Moreover, we analyze a special case - constant distortion function to provide more insights.

\subsection{Structure of the optimal policies}
\label{sec: main_res}
In this part, we first study the structure of the optimal policies, and then obtain the average cost function with regard to a threshold.

\begin{table*}[h]
\centering
\footnotesize
\caption{\small{Notations}}
\label{notations}
\begin{tabular}{l}
\hline\hline
$F(r)= \sum_{j=r}^{M}P_\Lambda(j), \ \ \forall \ 0\leq r\leq M$\\ \hline
$B_{l}=1-(1-p)F(h_l), \ \ \forall \ 1\leq l\leq L$\\ \hline
$w(i,j)=\mathbbm{1}_{\{i<j\}}\prod_{v=i}^{j-1}(B_{v})^{\delta_{v+1}-\delta_v}+\mathbbm{1}_{\{i\geq j\}}$
\\ \hline
 $J_{l}=-\frac{1}{(1-B_{{l}-1})^2}-\frac{\delta_{l}-1+\beta F(h_{{l}-1})}{1-B_{{l}-1}}$\\
 \ \ \ \ \ \ $+\sum_{j={l}}^{L}w({l},j)\Big(\frac{1-\mathbbm{1}_{\{j<L\}}(B_{j})^{\delta_{j+1}-\delta_j}\big(1+(\delta_{j+1}-1+\beta F(h_j))(1-B_j)\big)}{(1-B_j)^2}
    +\frac{\delta_j-1+\beta F(h_j)}{1-B_j}\Big), \ \ \forall \ 2\leq l\leq L$ 
 \\\hline $I_{l}=-\frac{1}{1-B_{{l}-1}}+\sum_{j={l}}^{L}\frac{1-\mathbbm{1}_{\{j<L\}}(B_{j})^{\delta_{j+1}-\delta_j}}{1-B_j}w(l,j), \ \ \forall \ 2\leq l\leq L$
 \\ \hline $O_{l}=\frac{1}{(1-B_{{l}-1})^2}+\frac{-1+\beta F(h_{{l}-1})}{1-B_{{l}-1}}, \ \ \forall \ 2\leq l\leq L+1$
 \\ \hline \hline
\end{tabular}
\vspace{-0.4cm}
\end{table*}

\begin{theorem}
\label{opt_stru}
For any fixed $\beta$, there exists an optimal age threshold $\Delta_\beta^\star$ such that the following policy $\pi_\beta^\star =(d_{\beta}^{\star},d_{\beta}^{\star},\cdots)$ where 
\begin{align}
&d_{\beta}^{\star}(\Delta,\Lambda)=
  \begin{cases}%{l l}  
  1 & \text{if}\, \, \Delta\geq \Delta_{\beta}^\star \, \ \text{and}\, \ \Lambda\geq D(\Delta),\\
  0 & \text{otherwise},
  \end{cases} \label{optPol}
\end{align}
achieves the minimum average Lagrangian cost in \eqref{avg_cost}. 
%Given $\beta$, there exists a stationary deterministic policy that solves problem \eqref{avg_cost}, which is in the form  $\pi_{\beta}^{\star}=(d_{\beta}^{\star},d_{\beta}^{\star},\cdots)$, where
%\begin{align}
%&d_{\beta}^{\star}(\Delta,\Lambda)=
 % \begin{cases}%{l l}  
%  1 & \text{if}\, \,\Delta_{\beta}^\star\leq \Delta\leq D^{-1}(\Lambda),\\
 % 0 & \text{otherwise},
 % \end{cases} \label{optPol}
%\end{align}
%where $\Delta_{\beta}^\star$ denotes the optimal threshold for the average cost MDP,
\end{theorem}
\begin{proof}
Please see Section \ref{proof_thre1}.
\end{proof}
By Theorem \ref{opt_stru}, the optimal policies for \eqref{avg_cost} are of threshold-type in the age. That is, if $D(\Delta_t)\!\!\!>\!\!\Lambda_t$, then the access point is not allowed to transmit due to the imposed maximum allowable distortion criterion. In the scenario  $D(\Delta_t)\!\leq\! \Lambda_t$,  the optimal policy would transmit if and only if the age $\Delta_t$ exceeds $\Delta_\beta^\star$. 
%Further, as long as the age exceeds the threshold and satisfies the distortion requirement, i.e., $\Delta\leq D^{-1}(\Lambda)$, it is optimal to transmit. Note that given $\Lambda_0$, if the threshold is larger than $D^{-1}(\Lambda_0)$ , then it is optimal to suspend transmission whenever $\Lambda_0$ samples are collected. 

Given a threshold, we can draw a state transition diagram under policy \eqref{optPol}, and obtain its average Lagrangian cost. In Theorem \ref{cost_cal}, we obtain the average cost as a function of threshold. 
\par Recall that $\delta_l$ is the leftmost point of the $l$-th interval in the distortion requirement function $D(\cdot)$, see Fig.~\ref{fig:distfun_inc} and Sec.~\ref{sec: const}. Given any $k\in\mathbb{N}^+$, define  
\begin{equation}
    l_k\triangleq \min\{l\leq L+1: \delta_l>k\}. \label{eqn:def_lk}
\end{equation}
Since per our definition $\delta_{L+1}=\infty$, we always have $l_k\leq L+1$. We then have the following results.  



\begin{theorem}
\label{cost_cal}
Using policy $\pi_k$ in the form of \eqref{optPol} with threshold $k\in\mathbb{N}^+$, the long-term average Lagrangian cost is expressed as:
\begin{footnotesize}
\begin{align}
   &\bar{L}(\pi_k;\beta) \notag\\
   =&\frac{0.5k^2-0.5k+(1-B_{{l_k}-1})^{-1}k
    +\mathbbm{1}_{\{l_k\leq L\}}J_{l_k} (B_{l_k-1})^{\delta_{l_k}-k}+O_{l_k}}{k-1+(1-B_{{l_k}-1})^{-1}
    +\mathbbm{1}_{\{l_k\leq L\}}I_{l_k} (B_{l_k-1})^{\delta_{l_k}-k}},\label{eqn:avg_cost}
\end{align}
\end{footnotesize}
for which the expressions of $\{B_{l}\}_{l=1}^L$, $\{J_{l}\}_{l=2}^L$, $\{I_{l}\}_{l=2}^L$, and $\{O_{l}\}_{l=2}^{L+1}$ are given in Table \ref{notations}.
\end{theorem}
\begin{proof-sketch}
With aid of the state transition diagram under the policy $\pi_k$, we obtain steady state probability of each state, which enables us to obtain the average cost $\bar{L}(\pi_k;\beta)$.
\end{proof-sketch}

The closed-form expression of $\bar{L}(\pi_k;\beta)$ allows us to search for the optimal threshold $k^\star$ numerically.  Unfortunately, the expression of \eqref{eqn:avg_cost} versus the threshold $k$ may exhibit complicated behavior (e.g., neither convex nor concave) and the domain of $k$ is unbounded.  To overcome these two challenges, we prove in the subsequent Theorem~\ref{new} that among the domain of $k\geq \delta_L$, we can analytically find the optimal $k_\text{UB}$.  Therefore, to search for the optimal $k^\star$, we only need to exhaustively evaluate $\bar{L}(\pi_k;\beta)$ for all $k\in \{1,2,\cdots,\delta_L-1\}$, compare their values to $\bar{L}(\pi_{k_\text{UB}};\beta)$ in Theorems~\ref{cost_cal} and~\ref{new}, and then find the globally minimum $k^\star$. Also see our discussion of low-complexity algorithm in Sec.~\ref{sec:alg_design}. 

\begin{theorem}
\label{new}
Among the sub-domain $k\geq \delta_L$, the $k$ that leads to the smallest $\bar{L}(\pi_k;\beta)$ is given by
\begin{align}
    k_\text{UB} &\triangleq \argmin_{k\geq \delta_L}\bar{L}(\pi_k;\beta)\\
    &=\max\{\delta_L,y\}, \label{eqn:k0}
\end{align}
where 
\begin{small}
\begin{align}
    y\!=\!\Bigg\lceil\!\!-\!\frac{1+B_L}{2(1-B_L)}\!+\!\left(\frac{B_L^2}{(1-B_L)^2}\!+\!\frac{B_L\!+\!2\beta F(h_L)}{1-B_L}\!+\!\frac{1}{4}\right)^{0.5}\!\Bigg \rceil.
\end{align}
\end{small}
\end{theorem}

\begin{proof-sketch}
To find the $k$ that minimizes $\bar{L}(\pi_k;\beta)$ among the sub-domain $k\geq \delta_L$, we show that $\bar{L}(\pi_k;\beta)$ either increases, or first decreases and then increases with $k$ on the sub-domain.
\end{proof-sketch}
%\vspace{0.05cm}

\subsection{Special Case - Constant Distortion}
\label{sec:special_case}
In this part, we consider a special case, where the distortion function is a constant function, i.e., $D(\Delta)=h\leq M$, $\forall \Delta$. Note that constant distortion function belongs to the set of non-decreasing distortion functions. Thus, the results in Section \ref{sec: main_res} hold for this special case.
Further, for the constant distortion function, $L\!=\!1$. By Theorem \ref{new}, we can directly obtain the optimal threshold. The results are summarized in the following corollary.

\begin{corollary}
\label{cor: special_case}
Given $\beta$ and constant distortion function $D(\Delta)=h$, there exists a stationary deterministic policy that solves problem \eqref{avg_cost}, which is in the form  $\pi_{\beta,\text{cons}}^{\star}=(d_{\beta,\text{cons}}^{\star},d_{\beta,\text{cons}}^{\star},\cdots)$, where
\begin{align}
&d_{\beta,\text{cons}}^{\star}(\Delta,\Lambda)=
  \begin{cases}%{l l}  
  1 & \text{if}\, \,\Delta\geq \Delta_{\beta,\text{cons}}^\star\, \ \text{and}\, \ \Lambda\geq D(\Delta),\\
  0 & \text{otherwise},
  \end{cases}
\end{align}
where the optimal threshold
$\Delta_{\beta,\text{cons}}^\star$ is given by 
\begin{footnotesize}
\begin{align}
    \Delta_{\beta,\text{cons}}^\star\!\! =
    \!\max\Bigg\{\!1,\!\Bigg\lceil\!\!-\!\frac{1+R}{2(1\!-\!R)}\!+\!\sqrt{ \!\frac{R^2}{(1\!-\!R)^2}\!+\!\frac{R\!+\!2\beta W}{1\!-\!R}\!+\!\frac{1}{4}}\Bigg \rceil\Bigg\},
    \label{opt_threval_spec}
\end{align}
\end{footnotesize}
where $W=\sum_{j=h}^{M}P_\Lambda(j)$ and $R=1-(1-p) W$.
\end{corollary}

\textbf{Remark:} By Corollary \ref{cor: special_case}, the optimal threshold $\Delta_{\beta,\text{cons}}^\star$ depends on Lagrangian multiplier $\beta$, distortion requirement $h$, the distribution on the number of collected samples $P_\Lambda(\cdot)$ and channel unreliability $p$. By simple algebraic simplification of \eqref{opt_threval_spec}, it is easy to show that when $\beta=0$, which corresponds to the case without energy constraint, we have $\Delta_{\beta,\text{cons}}^\star=1$. In addition, $\Delta_{\beta,\text{cons}}^\star$ is non-decreasing with $\beta$. This is because that the increase of $\beta$ implies higher weights of the energy cost. To save energy cost, the threshold should be increased to reduce the transmission frequency.

To provide more insights on the special case of constant distortion, we investigate how $W$ (determined by $h$, $P_\Lambda(\cdot)$) and $p$ affect the optimal threshold $\Delta_{\beta,\text{cons}}^\star$ in Theorem \ref{lem:special_case}.

\begin{theorem}
\label{lem:special_case}
Given $\beta>0$ and $D(\Delta)=h$, we have the following properties: 

(i) If $\beta >\frac{1}{W}$, the optimal threshold $\Delta_{\beta,\text{cons}}^\star$ is non-decreasing with $p$; if $\beta <\frac{1}{W}$, the optimal threshold $\Delta_{\beta,\text{cons}}^\star$ is non-increasing with $p$;

(ii) In fact, we can further strengthen the second half of (i) by the following: If $\beta <\frac{1}{W}$, the optimal threshold $\Delta_{\beta,\text{cons}}^\star=1$; 

(iii) The optimal threshold $\Delta_{\beta,\text{cons}}^\star$ is non-decreasing with $W$.
%(iv) The ratio of the resultant age cost and energy cost, i.e.,$\frac{\bar{A}(\pi_k)}{\bar{E}(\pi_k)}$ increases with the threshold.
\end{theorem}
\begin{proof-sketch}
Please see Appendix \ref{app: special_case}.
\end{proof-sketch}
\vspace{0.2cm}

\textbf{Remark}
Note that the Lagrangian multiplier $\beta$ can be viewed as the energy price of one transmission, and $\frac{1}{W}$ {\em is the expected duration between two consecutive slots when the distortion requirement is met}, which implies the age price of suspension. Then, the intuition of the theorem can be explained as follows:
\begin{itemize}
    \item 
In the case $\beta >\frac{1}{W}$, the energy cost matters. Then, as $p$ increases (channel worsens), the optimal threshold may be increased to save energy as stated in (i) of Theorem~\ref{lem:special_case}. In contrast, the age cost matters when $\beta <\frac{1}{W}$. Then, the optimal threshold needs to be decreased to obtain more transmission opportunities as $p$ increases.
\item For any $W$, if $p=0$ (reliable transmission from the access point to the receiver), then $\beta-\frac{1}{W}$ implies the instant cost of transmission minus the minimal instant cost of suspension. In the case, if $\beta-\frac{1}{W}<0$, then the optimal threshold is 1. Together with (i) that $\Delta^\star_{\beta,\text{cons}}$ is non-increasing with $p$ if $\beta<\frac{1}{W}$, we obtain (ii).
\item %Let $Y(k,W)\triangleq (\bar{E}(k,W)-\bar{E}(k+1,W))-(\bar{A}(k+1,W)-\bar{A}(k,W))$, where $\bar{E}(k,W)$ ($\bar{A}(k,W)$) denotes the resultant average energy (age) cost using $\pi_k$ given $W$.  Suppose given $W$, the optimal threshold is $k^\star$. Since the optimal policy should balance the energy savings and age increase, $Y(k^\star,W)\approx 0$. For $W<W'$, we have that $Y(k^\star,W)<Y(k^\star,W')$. Together with that $Y(k,W)$ is non-increasing with $k$, the optimal threshold may be increased to get a new balance at $W'$. This explains (iii).
The intuition of (iii) is as follows. For any given $\beta$, $W$, the optimal threshold $\Delta^\star_{\beta,\text{cons}}$ would perfectly balance the age cost and the energy cost in \eqref{avg_cost}. Consider a slightly larger $W'>W$. Since $\frac{1}{W}$ is the expected duration between two consecutive slots when the distortion requirement is met, the duration under $W'$ would be slightly smaller. The impact of having more chance to potentially transmit would increase the energy cost (since we send more frequently) and decrease the age cost (since we send more frequently). As a result, to re-balance the two, the optimal policy would further increase $\Delta^\star_{\beta,\text{cons}}$ under the new $W'$. 
\end{itemize}

%For the general non-decreasing case, we use simulations to investigate the impact of $q_m$, $p$ and $\beta$ on the optimal threshold in Section \ref{sec:simu1} and have similar observations.

\subsection{Proof of Theorem \ref{opt_stru}}
\label{proof_thre1}
A method to study average cost MDPs is to relate them to discounted cost MDPs. In this section, we (i) define discounted cost MDPs; (ii) obtain optimal policies for the discounted cost MDPs; and (iii) extend results to the average cost MDPs.

Given discount factor $\alpha \in (0, 1)$ and an initial state $\mathbf{s}$, the total expected discounted Lagrangian cost under policies $\pi\in\Pi$ is given by
\begin{align}
	&L_{\mathbf{s}}^{\alpha}(\pi;\beta)= \limsup_{T \rightarrow \infty} \mathbb{E}_{\pi}\big[\sum_{t=1}^T \alpha^{t-1}C(\mathbf{s}_{t},u_{t};\beta)|\mathbf{s}\big],
	\label{disc_cost0}
\end{align}

Then, the optimization problem of minimizing the total expected discounted Lagrangian cost while satisfying distortion requirement can be cast as

\textit{Problem 3 (Discounted cost MDP):}
\begin{equation}
	V^{\alpha}(\mathbf{s})\triangleq\min_{\pi\in\Pi} \ L_{\mathbf{s}}^\alpha(\pi;\beta),
	\label{disc_cost_opt_00}
\end{equation}
where $V^{\alpha}(\mathbf{s})$ denotes the optimal total expected $\alpha$-discounted Lagrangian cost (for convenience, we omit $\beta$ in $V^{\alpha}(\mathbf{s})$).

%A policy is said to be \emph{$\alpha$-discounted cost optimal} if it minimizes the total expected $\alpha$-discounted Lagrangian cost.
In Proposition \ref{existence_discount_00}, we introduce the optimality equation of $V^{\alpha}(\mathbf{s})$.
\begin{proposition}
\label{existence_discount_00}
	\noindent	(a) The optimal total expected $\alpha$-discounted Lagrangian cost, given by $V^{\alpha}(\Delta,\Lambda)$, satisfies the optimality equation as follows:
	\begin{align}
		V^{\alpha}\left(\Delta,\Lambda\right)=\min_{u\in A_{(\Delta,\Lambda)}}  Q^{\alpha}\left(\Delta,\Lambda;u\right), \label{opt_equ_disc_00}
	\end{align}	
	where
	\begin{align}
		Q^{\alpha}\left(\Delta,\Lambda;0\right)\!=&\Delta\!+\!\alpha \mathbb{E}V^{\alpha}\left(\Delta+1,\Lambda'\right);\label{q1_}\\
		%\displaybreak
		Q^{\alpha}\left(\Delta,\Lambda;1\right)\!=&\Delta\!+\!\beta
		\!+\!\alpha \Big(p \mathbb{E}V^{\alpha}\left(\Delta+1, \Lambda'\right)\notag\\
		&+\!(1\!-\!p)\mathbb{E}V^{\alpha}\left(1,\Lambda'\right)\Big).\label{q2_}
	\end{align}
	%\vspace{-0.1cm}
	
\noindent(b) A stationary deterministic policy determined by the right-hand-side of \eqref{opt_equ_disc_00} solves problem \eqref{disc_cost_opt_00}.% is $\beta$-discounted optimal. 
	
\noindent (c) Let $V_n^{\alpha}(\mathbf{s})$ be the cost-to-go function such that
$V_0^{\alpha}(\mathbf{s})\!=\!0$, for all $\mathbf{s}\in\mathcal{S}$ and for $n\geq 0$,
		\begin{align}
		V_{n+1}^{\alpha}(\Delta,\Lambda)=\min_{u\in A_{(\Delta,\Lambda)}} Q_{n+1}^{\alpha}(\Delta,\Lambda;u),
		\label{iteration00}
	    \end{align}
	    where
	    \begin{align}
		Q_{n+1}^{\alpha}\left(\Delta,\Lambda;0\right)=&\Delta+\alpha\mathbb{E} V_{n}^{\alpha}\left(\Delta+1,\Lambda'\right);\label{q1}\\
		Q_{n+1}^{\alpha}\left(\Delta,\Lambda;1\right)=&\Delta+\beta+\alpha \Big(p\mathbb{E} V_{n}^{\alpha}\left(\Delta+1, \Lambda'\right) \notag\\&+(1-p)\mathbb{E}V_{n}^{\alpha}
		\left(1,\Lambda'\right)\Big).\label{q2}
	    \end{align}
	    Then, we have $V_n^{\alpha}(\mathbf{s}) \rightarrow V^{\alpha}(\mathbf{s})$ as $n\rightarrow \infty$, $\forall \mathbf{s}, \alpha$.
\end{proposition}
\begin{proof-sketch}
By \cite{sennott1989average}, it suffices to show that there exists a stationary deterministic policy $f\in\Pi$ such that for all $\alpha$ and $\mathbf{s}$, we have $L_{\mathbf{s}}^\alpha(f;\beta)\!<\!\!\infty$. A policy that chooses $u=0$ at every time slot satisfies this.
%According to \cite{sennott1989average}, it suffices to show that there exists a stationary deterministic policy $f\in\Pi$ such that for all $\alpha$ and $\mathbf{s}$, we have $L_{\mathbf{s}}^\alpha(f;\beta)\!<\!\!\infty$.
%Let $f$ be a policy that chooses $u=0$ at every time slot. Obviously, $f$ satisfies the distortion constraint and thus $f\in\Pi$. Further, given the initial state $\mathbf{s}_1=(\Delta,\Lambda)$, we have 
%\begin{align}
%	L_{\mathbf{s}_1}^\alpha(f;\beta)&= \limsup_{T \rightarrow \infty} \mathbb{E}_f\big[\sum_{t=1}^T \alpha^{t-1}\Delta_t|\mathbf{s}_{1}\big]\\
%	&=\sum_{n=0}^{\infty}\alpha^n(\Delta+n)\\
%	&=\frac{\Delta}{1-\alpha}+\frac{\alpha}{(1-\alpha)^2}<\infty.
%\end{align}
\end{proof-sketch}

Using the induction method in (c) of Proposition \ref{existence_discount_00}, we first show some properties of $V^{\alpha}(\mathbf{s})$ in Lemma \ref{property_00}.
\begin{lemma}
\label{property_00}
Given $\alpha$, the value function $V^{\alpha}(\mathbf{s})$ has properties:

(i) The value function $V^{\alpha}(\mathbf{s})$ is non-decreasing with $\Delta$.

(ii) The value function $V^\alpha(\mathbf{s})$ is non-increasing with $\Lambda$.
\end{lemma}
\begin{proof-sketch}
By Proposition \ref{existence_discount_00}, $V_n^{\alpha}(\mathbf{s}) \!\!\rightarrow\!\! V^{\alpha}(\mathbf{s})$ as $n\rightarrow \infty$. Thus, we show that $V_n^{\alpha}(\mathbf{s})$ has (i) and (ii) for $n\in \mathbb{N}$. Obviously, $V_0^{\alpha}(\mathbf{s})$ has properties (i) and (ii) since $V_0^{\alpha}(\mathbf{s})=0$. Then, we show that given $V_n^{\alpha}(\mathbf{s})$ has the properties (i) and (ii), $V_{n+1}^{\alpha}(\mathbf{s})$ has these properties, $\forall n\geq 0$.
\end{proof-sketch}
\vspace{0.2cm}
%\begin{proof}
%Please see Appendix \ref{proof_prop_dis_subprob}.
%\end{proof}

Using the properties in Lemma \ref{property_00}, we further show that the optimal policies that solve discounted cost MDPs in \eqref{disc_cost_opt_00} are of threshold-type in Lemma \ref{disc_stru0}.
\begin{lemma}
\label{disc_stru0}
Given $\beta,\alpha$, the optimal policy that solves the discounted cost MDP \eqref{disc_cost_opt_00} is of threshold-type in the age. Specifically, there exists a threshold $\Delta_{\alpha,\beta}^{\star}$ such that it is optimal to transmit only when the age exceeds the threshold and the distortion requirement is met, i.e., $ \Delta\geq \Delta_{\alpha,\beta}^{\star} $ and $\Lambda\geq D(\Delta)$.
\end{lemma}
\begin{proof}
Please see Appendix \ref{proof_disc_stru}.
\end{proof}

 By \cite{sennott1989average}, under certain conditions (A proof of these conditions verification is provided in Appendix \ref{proof_cond}), the optimal policy for problem \eqref{avg_cost} can be viewed as a limit of a sequence of the optimal policies for the $\alpha$-discounted cost problems in \eqref{disc_cost_opt_00} as $\alpha\to 1$. Thus, there exist stationary deterministic policies that solve problem \eqref{avg_cost}, and the optimal policies are in the form \eqref{optPol}.
 
 


\section{Low-complexity Algorithm for average-age MDP}
\label{sec:alg_design}
In this section, we design a low-complexity algorithm for the average-age MDP. In particular, we first design a low-complexity algorithm to obtain the optimal policy for the average cost MDP \eqref{avg_cost} given $\beta$, and then provide a way to determine optimal Lagrangian multiplier $\beta$.
\subsection{Optimal policy for average cost MDP \eqref{avg_cost}}
In Theorem \ref{opt_stru}, we show that the optimal policy for \eqref{avg_cost} is of a threshold-type in the form of \eqref{optPol}. In order to obtain the optimal policy for \eqref{avg_cost}, it remains to obtain optimal threshold $\Delta_\beta^\star$. Using Theorems~\ref{cost_cal} and \ref{new}, we can find $\Delta_\beta^\star$ by the following Algorithm~\ref{alg0}. 
%Recall that in Theorem \ref{cost_cal}, we obtain the average cost under the threshold-type policy which is a piecewise function of the threshold. In addition, we obtain the threshold $k_0$ that minimizes the cost in the last interval of the domain. With this, we can find the optimal threshold by comparing the average costs of thresholds $k<H_L$ and $k_0$.

\begin{algorithm}
%\algsetup{linenosize=\small}
%\SetAlCapNameFnt{\footnotesize}
%\SetAlCapFnt{\footnotesize}
%\captionsetup[algorithm]{labelfont=footnotesize}
\caption{Optimal Threshold Calculator}
\label{alg0}    
\LinesNumbered
\footnotesize 
\textbf{Input:} $\{\delta_j\}_{j=1}^L$, $\{h_j\}_{j=1}^L$, $l=2$, $k^\star=\infty$, $\bar{L}^\star=\infty$, \;
\For{$k=1$ to $\delta_L$}{
\eIf{$k=\delta_L$}{
Calculate $k_\text{UB}$ using \eqref{eqn:k0} and $\bar{L}(\pi_{k_\text{UB}};\beta)$ using \eqref{eqn:avg_cost}\;
\If{$\bar{L}(\pi_{k_\text{UB}};\beta)<\bar{L}^\star$}{
$\bar{L}^\star=\bar{L}(\pi_{k_\text{UB}};\beta)$\, $k^\star=k_\text{UB}$\;}
}{
\If{$k=\delta_{l-1}$}{
Calculate $B_{l-1}$, $O_l$, $I_l$ and $J_l$ using Table \ref{notations}\;
$l=l+1$\;
}
Calculate $\bar{L}(\pi_k;\beta)$ using \eqref{eqn:avg_cost}\;
\If{$\bar{L}(\pi_k;\beta)<\bar{L}^\star$}{
$\bar{L}^\star=\bar{L}(\pi_{k};\beta)$\, $k^\star=k$\;}
}
}
\textbf{Output:} $k^\star$, $\bar{L}^\star$;
\end{algorithm}

\textbf{Remark:} Relative value iteration (RVI) is a classical way to solve the average cost MDP. However, RVI requires updating value functions of all states in each iteration. Since the state space is infinite in this problem, the state space would have to be truncated before applying RVI, which could introduce a significant error from the optimal solution. Compared with RVI, the advantage of the proposed algorithm \ref{alg0} is as follows:

(i) In Algorithm \ref{alg0}, we avoid dealing with infinite space. Instead, we compare average costs of threshold-type policies with \emph{finite} different thresholds.  %since we show the optimal policy is of threshold type, and we are able to determine optimal threshold on the domain $[H_L,\infty)$. 

(ii) In terms of complexity, each iteration of RVI takes $O(MX)$, where $X$ is the bound for the age and should be larger than $\delta_L$ to reduce offset from the optimal solution. However, Algorithm \ref{alg0} takes $O(\delta_L+M)$ to find optimal threshold /policy for \eqref{avg_cost}, which has less complexity than even two iterations of RVI.

\vspace{-0.5cm}
\subsection{Lagrangian multiplier estimate}
In Theorem \ref{Ori_Lag}, we have shown that the optimal policy for the average-age MDP \eqref{ori_prob} is a mixture of two stationary deterministic policies $\pi_{\beta^\star,1}$ and $\pi_{\beta^\star,2}$, each of which is optimal for the average cost MDP \eqref{avg_cost}. 

Our idea is to construct two sequences $\beta_n$ and $\beta_n'$ such that they satisfy
$\beta_n\leq \beta_n'$, $\beta_n \uparrow \beta^\star$ and $\beta'_n\downarrow \beta^\star$. By \cite{ceran2019average}, in practice, we can use optimal policies $\pi^\star_{\beta^-}$ and $\pi^\star_{\beta^+}$ to approximate policies $\pi_{\beta^\star,1}$ and $\pi_{\beta^\star,2}$, where $\beta^-\triangleq \beta_n$ and $\beta^+ \triangleq \beta'_n$ for reasonably large $n$; and $\pi^\star_{\beta^-}$ and $\pi^\star_{\beta^+}$ are optimal policies that solve \eqref{avg_cost} associated with $\beta^-$ and $\beta^+$, respectively. With $\beta^-$ and $\beta^+$, the randomization factor $\mu$ is calculated by
\begin{align}
\vspace{-0.5cm}
    \mu=\frac{E_\text{max}-\bar{E}(\pi^\star_{\beta^+})}{\bar{E}(\pi^\star_{\beta^-})-\bar{E}(\pi^\star_{\beta^+})},
    \label{mu_cal}
    \vspace{-0.3cm}
\end{align}
where $\bar{E}(\pi)$ is the average energy cost under policy $\pi$ as defined in \eqref{avg_energy}. Then, the optimal policy for the average-age MDP chooses $\pi^\star_{\beta^-}$ with probability $\mu$ and $\pi^\star_{\beta^+}$ with probability $1-\mu$ after each successful delivery.



In Algorithm \ref{alg1}, we provide a way to obtain parameters $\beta^+$, $\beta^-$ and $\mu$, which determines the optimal policy for the average-age MDP \eqref{ori_prob}. In particular, we use bisection method to obtain $\beta^-$ and $\beta^+$ that follows the methodology in \cite{sennott1993constrained}. 
In Algorithm~\ref{alg1}, the expression of the average energy cost with a threshold $k$ is 
\begin{small}
\begin{align}
    &\bar{E}(\pi_k)=\Bigg\{\frac{ F(h_{{l_k}-1})}{1-B_{{l_k}-1}}+\mathbbm{1}_{\{l_k\leq L\}}(B_{{l_k}-1})^{\delta_{l_k}-k}\bigg(-\frac{ F(h_{{l_k}-1})}{1-B_{{l_k}-1}}\notag\\
   % \displaybreak
    &+\sum_{j=l_k}^{L}w(l_k,j) F(h_j)\frac{1-\mathbbm{1}_{\{j<L\}}(B_{j})^{\delta_{j+1}-\delta_j}}{1-B_j}\bigg)\Bigg\}z^{-1},
    \label{avg_cost_cal}
\end{align}
\end{small}
where $z=k-1+(1-B_{{l_k}-1})^{-1}+\mathbbm{1}_{\{l_k\leq L\}}I_{l_k} (B_{{l_k}-1})^{\delta_{l_k}-k}$ and $l_k$ is defined previously in \eqref{eqn:def_lk}. The derivation of \eqref{avg_cost_cal} is part of the proof of Theorem \ref{cost_cal}.

\begin{algorithm}
%\algsetup{linenosize=\small}
%\SetAlCapNameFnt{\footnotesize}
%\SetAlCapFnt{\footnotesize}
%\captionsetup[algorithm]{labelfont=footnotesize}
\caption{Low-complexity Optimal Transmission Scheduler Estimator}
\label{alg1}    
\LinesNumbered
\footnotesize 
\textbf{Input:} $\epsilon>0$, $\beta^{-}$, $\beta^{+}$ \;
\While{$|\beta^+-\beta^-|>\epsilon$}{
$\beta=(\beta^++\beta^-)/2$\;
For the new $\beta$, obtain optimal threshold $k^\star$using Algorithm~\ref{alg0}\;
Calculate average energy cost using \eqref{avg_cost_cal}\;
 \eIf{$\bar{E}(\pi_{k^\star})>E_{\text{max}}$}{
 $\beta^-=\beta$\;}{
 $\beta^+=\beta$\;
 }
 }
 Compute $\mu$ using \eqref{mu_cal}\;
\textbf{Output:} $\mu$, $\beta^+$ and $\beta^-$\;
\end{algorithm}

%\vspace{-0.2cm}
\section{Simulations}
\label{sec:simu}
In this section, we numerically evaluate the performance of
the proposed algorithms.
\subsection{Optimal threshold for problem \eqref{avg_cost}}
\label{sec:simu1}
To provide more insights, we investigate how the optimal threshold varies with $\beta$ and error probabilities, respectively. 
\subsubsection{Constant distortion requirement}
We first simulate the special case. In simulation, we set $h=5$, $M=10$ and $q_m=q$, $\forall m$. Fig. \ref{fig:opt_thre_f} studies the optimal threshold versus $W$ given $p=0.5$ and $\beta \in\{5,10,20\}$, where $W$ is changed by changing $q$. From Fig. \ref{fig:opt_thre_f}, we observe that the optimal threshold increases with $W$. Fig. \ref{fig:opt_thre_p} studies the optimal threshold versus $p$ given $\beta=10$ and $W\in\{0.03,0.36,0.83\}$. From Fig. \ref{fig:opt_thre_p}, we observe that the optimal threshold increases with $p$ for $W=0.36$ or $W=0.83$ ($\beta>\frac{1}{W}$). Moreover, for all cases in Figs. \ref{fig:opt_thre_f} and \ref{fig:opt_thre_p} that satisfy $\beta<\frac{1}{W}$, the optimal threshold is one. These observations confirm our theoretical results in Theorem~\ref{lem:special_case}.
\begin{figure}[H]
\vspace{-0.2cm}
    \centering
    \includegraphics[width=0.42\textwidth]{specCase_optThre_W.eps}
    \caption{Optimal threshold $\Delta^\star_{\beta,\text{cons}}$ vs $W$ given $p=0.5$}
    \label{fig:opt_thre_f}
    \vspace{-0.2cm}
\end{figure}  

\begin{figure}
    \centering
    \includegraphics[width=0.42\textwidth]{specCase_optThre_p.eps}
    \caption{Optimal threshold $\Delta^\star_{\beta,\text{cons}}$ vs $p$ given $\beta=10$}
    \label{fig:opt_thre_p}
   \vspace{-0.5cm}
\end{figure} 

\subsubsection{Non-decreasing age-vs-distortion requirement}
For general non-decreasing distortion function, we set $M=8$, $L=3$, and $q_m=q$, $\forall m$. The distortion function is given by $\delta_1=1, \delta_2=25, \delta_3=50$ and $h_1=2, h_2=5, h_3=7$. Also see Fig.~\ref{fig:distfun_inc}. 




 

With this, we obtain the optimal threshold for different $\beta\in \{5, 25, 45\}$, and error probabilities $p\in \{0.1, 0.2,\cdots 0.9\}$ and $q \in \{0.1, 0.2,\cdots 0.9\}$ using Algorithm \ref{alg0}.
The results are summarized in Fig. \ref{fig:OptThre}.
In each sub-figure of Fig. \ref{fig:OptThre}, we investigate the impact of $p$ and $q$ on the optimal threshold. On one side, we observe that the optimal threshold decreases with $q$. This is consistent with the analysis result in the constant $D(\cdot)$ case in Sec.~\ref{sec:special_case} even though we do not have any analytical proof of this phenomenon. The intuition is that the increase of $q$ will reduce the probability that the distortion requirement is satisfied. This increases the demand for more transmission opportunities to maintain low age, which reduces the optimal threshold. On the other side, we observe that the optimal threshold either increases or deceases or first increases and then decreases with $p$ (see $q=0.6$ in Figs.~\ref{fig:thre_beta5},~\ref{fig:thre_beta25}, and \ref{fig:thre_beta45}). Whether the optimal threshold increases with $p$ depends on whether the age or the energy cost is the dominant issue, also see our discussion right after Theorem~\ref{new}. In particular, when the dominant issue to deal with is the energy cost, the optimal threshold increases with $p$. This is because increasing $p$ implies increasing energy consumption for a successful update. To save energy, the optimal threshold is increased. When the dominant issue to deal with is the age, the optimal threshold decreases with $p$. This is because that the increase of $p$ implies that more transmission attempts are needed for a successful delivery. To keep the age low, the optimal threshold should be reduced to provide more transmission opportunities.

Moreover, comparing Figs. \ref{fig:thre_beta5}, \ref{fig:thre_beta25} and \ref{fig:thre_beta45}, we observe that the optimal threshold increases with $\beta$. This is because as $\beta$ increases, more weights are placed on the energy cost, which requires increasing the threshold to reduce the energy cost.
\ifreport
 \begin{figure*}[]
 \centering
 \subfloat[$\beta=5$]{
 \includegraphics[scale=.35]{Age_dist/OptThre_N8_beta5.eps}
 \label{fig:thre_beta5}
 }\ 
 \subfloat[$\beta=25$]{
 \includegraphics[scale=.35]{Age_dist/OptThre_N8_beta25.eps}
 \label{fig:thre_beta25}
 }\\  
 %
 \subfloat[$\beta=45$]{
 \includegraphics[scale=.35]{Age_dist/OptThre_N8_beta45.eps}
 \label{fig:thre_beta45}
 }
 \caption{The optimal threshold $\Delta_\beta^\star$ vs transmission error probabilities with different values of $\beta$}
 \label{fig:OptThre}
\end{figure*}
\else
\begin{figure*}[]
 \subfloat[$\beta=5$]{
 \includegraphics[scale=.28]{OptThre_N8_beta5.eps}
 \label{fig:thre_beta5}
 }\ 
 \subfloat[$\beta=25$]{
 \includegraphics[scale=.28]{OptThre_N8_beta25.eps}
 \label{fig:thre_beta25}
 }\  
 \subfloat[$\beta=45$]{
 \includegraphics[scale=.28]{OptThre_N8_beta45.eps}
 \label{fig:thre_beta45}
 }
 \caption{The optimal threshold $\Delta_\beta^\star$ vs transmission error probabilities with different values of $\beta$}
 \label{fig:OptThre}
      \vspace{-0.5cm}
\end{figure*}
\fi 

\vspace{-0.2cm}
\subsection{Comparison with greedy policy}
Let $e_t$ denote the total energy consumption before the time slot $t$. Then, $\bar{e}_t=e_t/(t-1)$ denotes the average energy cost consumed before $t$. In this part, we compare the Algorithm \ref{alg1} with a greedy policy which transmits 
whenever transmission is allowed (i.e., $\Lambda\geq D(\Delta)$) and if the empirical energy cost is less than the energy budget (i.e., $\bar{e}_t<E_\text{max}$). 
%whenever $\Lambda\geq D(\Delta)$ and $\bar{e}_t<E_{\text{max}}$. 
The setting is same as in 2) of \ref{sec:simu1}. 
\ifreport
\begin{figure}
    \centering
    \includegraphics[width=0.65\textwidth]{Age_dist/comp_greedy.eps}
    \caption{Average age vs energy constraint $E_{\text{max}}$ using the proposed policy (Algorithm \ref{alg1}) and greedy policy}
    \label{fig:comp_greedy}
\end{figure}
\else
\begin{figure}
 \vspace{-0.2cm}
    \centering
    \includegraphics[width=0.43\textwidth]{comp_greedy.eps}
    \caption{Average age vs energy constraint $E_{\text{max}}$ using the proposed policy (Algorithm \ref{alg1}) and greedy policy}
    \label{fig:comp_greedy}
         \vspace{-0.6cm}
\end{figure}
\fi 

In Fig. \ref{fig:comp_greedy}, we observe that under either policy, the average age decreases with $E_{\text{max}}$. Moreover, Algorithm \ref{alg1} outperforms the greedy policy, and the gap between Algorithm \ref{alg1} and the greedy policy is the largest when under a tight energy constraint (small $E_\text{max}$). 

==> structure_algo.tex <==
\section{Structure of Average-Optimal Policy and Algorithm Design}
\label{structure}
In this section, we investigate the structure of the average-optimal policy and propose an efficient algorithm for the original problem \eqref{equiv1}.
\subsection{Threshold Structure of Average-Optimal Policy}
\label{struc}
\subsubsection{Threshold structure:}
The following theorem states that there exists a threshold-type stationary deterministic policy that is average-optimal. In particular, the problem is divided into two cases based on the relation between $d_1(1-p_2)$ and $d_2(1-p_1)$. Under these two cases, the threshold-type average-optimal policy shows opposite behaviors. 
\begin{theorem}
\label{THRE_PROP}
There exists a stationary deterministic average-optimal transmission selection policy that is of threshold-type. Specifically,

\noindent(i) If $d_1(1-p_2)\leq d_2(1-p_1)$, then the average-optimal policy is of the form $\pi^*=(\zeta^*,\zeta^*,\cdots)$, where
\begin{align}
\label{type2}
 &\zeta^*(a)=
  \begin{cases}%{l l}  
  2 & \text{if}\, \, 0\leq a\leq a_1^*, \\
  1 & \text{if} \, \,a_1^*< a,
  \end{cases} %\right.		
\end{align}
where $a_1^*$ denotes the age threshold.

\noindent(ii) If $d_1(1-p_2)\geq d_2(1-p_1)$, then the average-optimal policy is of the form $\pi^*=(\zeta^*,\zeta^*,\cdots)$, where
\begin{align}
\label{type1}
 &\zeta^*(a)=
  \begin{cases}%{l l}  
  1 & \text{if}\, \, 0\leq a\leq a_2^*, \\
  2 & \text{if} \, \,a_2^*< a,
  \end{cases} %\right.		
\end{align}
where $a_2^*$ denotes the age threshold.


\end{theorem}
\begin{proof}
	Please see Section \ref{proof}.
\end{proof}

Define the mean delay of transmission mode $j\in\mathcal{U}$ as 
\begin{align}
	\bar{d}_j\triangleq\frac{d_j}{1-p_j}.
	\label{mean_delay}
\end{align}
By Theorem \ref{THRE_PROP} (i), when the age exceeds a certain threshold, the optimal policy chooses the transmission with smaller mean delay. This result reveals an interesting phenomenon: While the transmission with minimum mean delay is the optimal decision for minimizing the average delay, this does not necessarily minimize the age.  
In particular, when the age is below a certain threshold, the average age is reduced by choosing a faster transmission that has a higher mean delay (i.e., a higher error probability). The reason is that if successful, the age remains low. If it fails, it provides an opportunity to generate a later packet that can be transmitted in a shorter period of time.
 %In addition, when age is below certain threshold, optimal policy chooses slow transmission under condition $d_1(1-p_2)\geq d_2(1-p_1)$ but fast transmission under condition $d_1(1-p_2)\leq d_2(1-p_1)$. This can be explained as follows: Condition $d_1(1-p_2)\geq d_2(1-p_1)$ can be rewritten as $\frac{d_1}{d_2}\geq \frac{1-p_1}{1-p_2}$, which implies that the gap between delays are larger than reliabilities. In other words, delays play an more important role. Thus, it is optimal to choose fast
In Section \ref{alg}, based on Theorem \ref{THRE_PROP} (ii), we will show that the averge-optimal policy under $d_1(1-p_2)\geq d_2(1-p_1)$ is to choose high rate transmission for each transmission opportunity. This is reasonable because both the delay and mean delay (including the impact of the error probability) of high rate transmission is shorter than that of low rate transmission.

\subsubsection{Proof of Theorem \ref{THRE_PROP}}
\label{proof}
One way to investigate the average cost MDPs is to relate them to the discounted cost MDPs. To prove Theorem \ref{THRE_PROP}, we (i) address a discounted cost MDP, i.e., establish the existence of a stationary deterministic policy that solves the MDP and then study the structure of the optimal policy; and (ii) extend the results to the average cost MDP problem in \eqref{avg_prob}.

Given an initial state $a$, the total expected $\alpha$-discounted cost under a transmission selection policy $\pi\in \Pi$ is given by 
\begin{align}
	V^\alpha(a;\pi)=\limsup_{n\rightarrow\infty}\mathbb{E}\left[\sum_{i=0}^{n-1}\alpha^i C(a_i,u_i)\right],
	\label{disc_cost}
\end{align}
where $0<\alpha<1$ is the discount factor. Then, the optimization problem of minimizing the total expected $\alpha$-discounted cost can be cast as

\emph{Problem 2 (Discounted cost MDP)} 
\begin{align}
	V^\alpha(a)\triangleq\min_{\pi\in \Pi} V^\alpha(a;\pi),
	\label{disc_prob}
\end{align} 
where $V^\alpha(a)$ denotes the optimal total expected $\alpha$-discounted cost. A transmission selection policy is said to be \emph{$\alpha$-discounted cost optimal} if it solves the problem in \eqref{disc_prob}. In Proposition \ref{DISC_EXIST}, we show that there exists a stationary deterministic transmission selection policy which is $\alpha$-discounted cost optimal and provide a way to explore the property of the optimal policy.

\begin{proposition}
\label{DISC_EXIST}
(a) The optimal total expected $\alpha$-discounted cost $V^\alpha$ satisfies the following optimality equation:
\begin{align}
	V^\alpha(a)=\min_{u\in \mathcal{U}} Q^\alpha(a, u),
	\label{bellman_equ}
\end{align}
where 
\begin{align}
	Q^\alpha(a, u)=C(a,u)+\alpha p_uV^\alpha(a+d_u)+\alpha(1-p_u)V^\alpha(d_u).
	\label{qvalue}
\end{align}

(b) The stationary deterministic policy determined by the right-hand-side of \eqref{bellman_equ} is $\alpha$-discounted cost optimal.

(c) Let $V_n^\alpha(a)$ be the cost-to-go function such that $V_0^\alpha(a)=\frac{d_1-d_2}{\alpha(p_2-p_1)}a$ and for $n\geq0$
\begin{align}
	V_{n+1}^\alpha(a)=\min_{u\in \mathcal{U}} Q_{n+1}^\alpha(a, u),
	\label{value_iter}
\end{align}
where
\begin{align}
	Q_{n+1}^\alpha(a, u)=C(a, u)+\alpha p_uV_n^\alpha(a+d_u)+\alpha(1-p_u)V_n^\alpha(d_u).
\end{align}
Then, we have that for each $\alpha$, $V_{n}^\alpha(a)\rightarrow V^\alpha(a)$ as $n\rightarrow \infty$.
\end{proposition}
%\begin{proof}
%Please see Appendix \ref{proposition}.
%\end{proof}
 \ifreport
\begin{proof}
See Appendix \ref{proposition}.
\end{proof}
\else 
\begin{proof}
See our technical report \cite{yao2020age}.
\end{proof}
\fi

Next, with the optimality equation \eqref{bellman_equ} and value iteration \eqref{value_iter}, we show that the optimal policy is of threshold-type in Lemma \ref{THRESHOLD}.


\begin{lemma} \label{THRESHOLD}
Given a discount factor $\alpha$,

(i) if $(1-\alpha p_2)d_1\leq (1-\alpha p_1)d_2$, then the $\alpha$-discounted cost optimal policy is of threshold-type, i.e., the optimal action is a non-increasing function of the age.%$\zeta_\alpha^*(a)=1$ if and only if age $a$ is larger or equal to some threshold.

(ii) if $(1-\alpha p_2)d_1\geq (1-\alpha p_1)d_2$, then the $\alpha$-discounted cost optimal policy is of threshold-type, i.e., the optimal action is a non-decreasing function of the age. %$\zeta_\alpha^*(a)=2$ if and only if age $a$ is larger or equal to some threshold;


\end{lemma}

\begin{proof}
Please see Appendix \ref{discount_threshold}
\end{proof}

This lemma proves that the $\alpha$-discounted cost optimal policy is of threshold-type. Next, we extend the results to average cost MDP and show that there exists a stationary deterministic average-optimal policy which is of threshold-type. Based on the results in \cite{sennott1989average}, we have the following lemma, which provides a candidate for average-optimal policy.
\begin{lemma}
\label{CANDI}
	(i) Let $\alpha_n$ be any sequence of discount factors converging to 1 with $\alpha_n$-discounted cost optimal stationary deterministic policy $\pi^{\alpha_n}$. There exists a subsequence $\gamma_n$ and a stationary policy $\pi^*$ that is a limit point of $\pi^{\gamma_n}$. 
	
	(ii) If $d_1(1-p_2)\leq d_2(1-p_1)$, $\pi^*$ is of threshold-type in \eqref{type2}; if $d_1(1-p_2)\geq d_2(1-p_1)$, $\pi^*$ is of threshold-type in \eqref{type1}.
\end{lemma}
\ifreport
\begin{proof}
See Appendix \ref{candidate_policy}.
\end{proof}
\else 
\begin{proof}
See our technical report \cite{yao2020age}.
\end{proof}
\fi


\ifreport
By \cite{sennott1989average}, under certain conditions (A proof of these conditions verification is provided in Appendix \ref{app1}), $\pi^*$ is average-optimal.  
\else 
By \cite{sennott1989average}, under certain conditions (A proof of these conditions verification is provided in our technical report \cite{yao2020age}), $\pi^*$ is average-optimal.
\fi

\subsection{Algorithm Design}
\label{alg}
Recall that if $p(\beta)=0$, then the optimal transmission selection policies that solve \eqref{equiv1} and \eqref{equiv2} are identical. Given $\beta$, the optimal policy that solves \eqref{equiv2} is of threshold-type by Theorem \ref{THRE_PROP} and then \eqref{equiv2} can be re-expressed as
\begin{numcases}{p(\beta)=}
\min_{\pi \in \Pi_1} J(\pi,\beta), & if $d_1(1-p_2)< d_2(1-p_1)$\label{pBeta2}\\
\min_{\pi \in \Pi_2} J(\pi,\beta), & if $d_1(1-p_2)\geq d_2(1-p_1)$\label{pBeta1}
\end{numcases}
where $\Pi_1$ and $\Pi_2$ denote the sets of threshold-type policies in \eqref{type2} and \eqref{type1}, respectively. 
Thus, the optimal policy that solves \eqref{equiv1} can be obtained with two steps: 
\begin{itemize}
	%\item (i) for each $\beta$ and threshold-based policy $\pi$, we obtain the expression of $J(\pi,\beta)$ in \eqref{avg_cost};
	\item \textbf{Step (i):} For each $\beta$, find the $\beta$-associated average-optimal policy $\pi^*_\beta$ such that $p(\beta)=J(\pi^*_\beta,\beta)$. 	
\item \textbf{Step (ii):} Find $\beta^*$ such that $p(\beta^*)=0$. This implies $\pi^*_{\beta^*}$ solves \eqref{equiv1}. 
\end{itemize}
To narrow our searching range in (ii), in Lemma \ref{BETA_RANGE}, we provide a lower bound $\beta_\text{min}$ and an upper bound $\beta_\text{max}$ of $\beta^*$. Then, for (i), we only need to pay attention to $p(\beta)$ for $\beta\in[\beta_\text{min},\beta_\text{max}]$. 

In particular, within the range of $\beta$, we show that $J$ in \eqref{pBeta2} is \emph{quasi-convex} in a threshold related variable, which enables us to devise a \emph{low-complexity} algorithm based on golden section search. Moreover, we show that $\pi^*_\beta$ that solves \eqref{pBeta1} always chooses $u=2$, which allows us to get the optimal policy for \eqref{equiv1} directly. 
 
\begin{lemma}
\label{BETA_RANGE}
	The parameter $\beta^*$ is lower bounded by $\beta_\text{min}\triangleq 1.5d_2$ and upper bounded by $\beta_\text{max}\triangleq\min\Big\{(\frac{1}{1-p_1}+0.5)d_1,(\frac{1}{1-p_2}+0.5)d_2\Big\}$.
\end{lemma}
%\begin{proof}
%	Please see Appendix \ref{range}.
%\end{proof}
\ifreport
\begin{proof}
See Appendix \ref{range}.
\end{proof}
\else 
\begin{proof}
See our technical report \cite{yao2020age}.
\end{proof}
\fi

In the following content, we provide a theoretical analysis step by step for our algorithm design in Algorithm \ref{alg1}, which returns the optimal threshold and optimal average age for \eqref{equiv1}. %In particular, within the range of $\beta^*$ obtained in Lemma \ref{BETA_RANGE}, we show that the cost function is convex or quasi-convex in a threshold related variable, which is used 

\begin{algorithm}[]
\caption{Threshold-based Age-Optimal Policy}
\label{alg1}
\LinesNumbered
\footnotesize
given $d_1$, $d_2$, $p_1$, $p_2$,$\tau=(\sqrt{5}-1)/2$, tolerance $\epsilon_1$, $\epsilon_2$, $l=\beta_\text{min}$, $r=\beta_\text{max}$\;
\While {$r-l>\epsilon_1$}{	
 $\beta=\frac{r+l}{2}$\;
 \eIf{$d_1(1-p_2)\geq d_2(1-p_1)$}{
 $m=0$, $k=0$, $J^*=J_2(0,0,\beta)$\;}
 {
 $k_\text{max}=\lfloor\frac{d_1}{d_2}\rfloor$, $J^*=f(1,0,\beta)$\;
	\ForEach{ $k_1\in \{0,1,\cdots,k_\text{max}\}$ }{		
		\eIf{$\frac{\partial J_1(y, k_1,\beta)}{\partial y}\vert_{y=1}<0$}{
			$m=0$\;
			}{
		$y_0=0$, $y_1=1$, $y_2=y_1-(y_1-y_0)\tau$, $y_3=y_0+(y_1-y_0)\tau$\;
		\While{$p_2y_1 \geq y_0$ and $y_1-y_0>\epsilon_2$}{
			\eIf{$J_1(y_2,k_1,\beta)>J_1(y_3,k_1,\beta)$}{
			$y_0=y_2$\;
			}{
			$y_1=y_3$\;
			}
			$y_2=y_1-(y_1-y_0)\tau$, $y_3=y_0+(y_1-y_0)\tau$\;
		}
		$t_1=\lfloor\log_{p_2} y_0\rfloor$, $t_2=\lceil\log_{p_2} y_1\rceil$\;
		$m=\argmin_{m\in\{t_1,t_2\}} J_1({p_2}^{m};k,\beta)$\;
		}		
	 \If{$J_1(p_2^{m}, k_1,\beta)\leq J^*$}{
	 $J^*=J_1(p_2^{m}, k_1,\beta)$\;
	}	
	}
	}	
	\eIf{$J^*\geq0$}{
 			$l=\beta$\;}{
 			$r=\beta$\;
		}
		
}
\end{algorithm}

\textbf{Step (i): Find the optimal policy $\pi^*_\beta$:}
%Let $a^*\in \mathbb{R}$ denote the age threshold of the threshold-type policy. 
%To find $\pi^*_\beta$, we first obtain the expression of $J(\pi,\beta)$ under threshold-type policies.
Note that both of the threshold-type policies defined in \eqref{type2} and \eqref{type1} result in a Markov chain with a single positive recurrent class. Thus, given threshold $a_1^*$ in \eqref{type2} or $a_2^*$ in \eqref{type1}, we can obtain the expression of average cost under the corresponding threshold-type policy with aid of state transition diagram. With this, we obtain some nice properties of average cost function in Theorem \ref{CONVEXITY}, which enables us to get a low-complexity algorithm. Before providing the result, we define the integer threshold which will be used in the theorem and algorithm.

Recall that age $a\in \mathcal{S}$ is expressed as the sum of multiple $d_1$'s and $d_2$'s. 
Note that under the threshold-type policy in \eqref{type2}, if $ a\leq a_1^*$, $\zeta(a)=2$. This implies that if $ a\leq a_1^*$, $a$ is in the form $a=d_j+l d_2, j\in\mathcal{U}, l\in \mathbb{N}$. Thus, it is sufficient to use the following integer threshold to represent the threshold-type policy in \eqref{type2}.
\begin{align}
	m_1&\triangleq\min \left\{l: d_1+ld_2> a_1^*,l \in  \mathbb{N}\right\},\label{3}\\
	n_1&\triangleq\min \left\{l: d_2+ld_2> a_1^*,l \in  \mathbb{N} \right\}\label{4}.
\end{align}
With this, the threshold policy in \eqref{type2} is rewritten as
\begin{align}
 &\zeta^*(a)=
  \begin{cases}%{l l}  
  2 & \text{if}\, \,  a< d_1+m_1d_2\ \ \text{and}\ \ a< d_2+n_1d_2, \\
  1 & \text{if} \, \,a\geq d_1+m_1d_2\ \ \text{or}\ \ a\geq d_2+n_1d_2.
  \end{cases} %\right.		
  \label{new_type2}
\end{align}
Similarly, the policy in \eqref{type1} can be rewritten as
\begin{align}
 &\zeta^*(a)=
  \begin{cases}%{l l}  
  1 & \text{if}\, \,  a< d_1+m_2d_1\ \ \text{and}\ \ a< d_2+n_2d_1, \\
  2 & \text{if} \, \,a\geq d_1+m_2d_1\ \ \text{or}\ \ a\geq d_2+n_2d_1,
  \end{cases} %\right.		
  \label{new_type1}
\end{align}
where
\begin{align}
m_2&\triangleq\min \left\{l: d_1+ld_1> a_2^*, l \in \mathbb{N}\right\},\label{1}\\
	n_2&\triangleq\min \left\{l: d_2+ld_1> a_2^*, l \in \mathbb{N} \right\}\label{2}.
\end{align}

Based on the analysis, \eqref{pBeta2} and \eqref{pBeta1} can be re-expressed as
\begin{numcases}{p(\beta)=}
\min_{m_1, k_1} J_1(m_1, k_1,\beta), \! & \!if $d_1(1-p_2)\!\!<\! d_2(\!1-p_1\!)$ \label{target2}\\
\min_{m_2, k_2} J_2(m_2, k_2,\beta),\! & \!if $d_1(1-p_2)\!\!\geq \!d_2(\!1-p_1\!)$ \label{target1}
\end{numcases}
%\begin{align}
%	p(\beta)\!\!\triangleq \!
%  \begin{cases}%{l l}  
%  \min_{m_2, k_2} J_2(m_2, k_2,\beta),\! & \text{if}\, \, d_1(1-p_2)\!\geq d_2(1-p_1), \\
%  \min_{m_1, k_1} J_1(m_1, k_1,\beta),\! & \text{if} \, \,d_1(1-p_2)\!< d_2(1-p_1),
%  \end{cases} 
%  \label{target}
%\end{align}
where $k_1=n_1-m_1$ and $k_2=n_2-m_2$. Also, we use $J_1(m_1, k_1,\beta)$ and $J_2(m_2, k_2,\beta)$ to denote the average cost under the policies in \eqref{new_type2} and \eqref{new_type1}, respectively. We have $k_2\in \mathcal{K}_2\triangleq\{0,1\}$ and $k_1\in \mathcal{K}_1\triangleq\big\{0,\cdots,\lfloor\frac{d_1}{d_2}\rfloor\big\}$. In particular, according to the definition of $m_2$ and $n_2$, we have $(m_2+1)d_1>a_2^*\geq d_2+(n_2-1)d_1$ and $d_2+n_2d_1>a_2^*\geq m_2d_1$. Substitute $k_2=n_2-m_2$ into these two inequalities, we get $k_2\in \mathcal{K}_2$. Similarly, we have $k_1\in \mathcal{K}_1$.

%Let $k_2=n_2-m_2$ and $k_1=n_1-m_1$. According to the definition of $m_2$ and $n_2$, we have $(m_2+1)d_1\geq a^*>d_2+(n_2-1)d_1$ and $d_2+n_2d_1\geq a^*>m_2d_1$. Substitute $k_2=n_2-m_2$ into these two inequalities and we have $k_2\in \mathcal{K}_2\triangleq\{0,1\}$. Similarly, we have $k_1\in \mathcal{K}_1\triangleq\big\{0,\cdots,\lfloor\frac{d_1}{d_2}\rfloor\big\}$.
%Note that if $d_1(1-p_2)\geq d_2(1-p_1)$ holds, then every threshold $a^*$ corresponds to a pair of $m_2$ and $k_2$. Thus, given $\beta$, we can obtain $p(\beta)$ by searching through all possible pairs of $m_2$ and $k_2$. That is, 
%\begin{align}
%p(\beta)=\min_{m_2, k_2} J_2(m_2, k_2,\beta),
%\label{target1}
%\end{align}
%where $J_2(m_2, k_2,\beta)$ denotes the average cost under the policy in \eqref{type1} with integer threshold $m_2$ and $k_2$. 
%Similarly, if $d_1(1-p_2)< d_2(1-p_1)$ holds, then the $p(\beta)$ is obtained by
%\begin{align}
%p(\beta)=\min_{m_1, k_1} J_1(m_1, k_1,\beta),
%\label{target2}
%\end{align}
%where $J_1(m_1, k_1,\beta)$ denotes the average cost under the policy in \eqref{type2} with integer threshold $m_1$ and $k_1$. 
%In Table \ref{notations}, we define some notations, which will be used in the expression of $J_2(m_2, k_2,\beta)$ and $J_1(m_1, k_1,\beta)$ in Lemma \ref{AVG_COST_THRED}.
\begin{table}[]
\renewcommand\arraystretch{2}
\caption{Notations}
\footnotesize
\begin{tabular}{p{0.8mm}l}
\hline\hline
$A_1$&$= p_2^{k_1}\big(d_2(1-p_1)-d_1(1-p_2)\big)\big(d_2(k_1+1)-d_1\big)$ \\
\hline
$B_1$&$= -A_2+p_2^{k_1}(1-p_2)(0.5d_1^2-\beta d_1+\frac{d_1^2}{1-p_1})+(1-p_1)(\beta d_2-0.5d_2^2-\frac{d_2^2}{1-p_2})$ \\
\hline
$C_1$&$= (1-p_1)(0.5d_2^2-\beta d_2+\frac{1}{1-p_2})d_2^2$ \\
\hline
$D_1$&$= \big(d_1(1-p_2)-d_2(1-p_1)\big)d_2p_2^{k_1}$\\
\hline
$A_2$&$= p_1^{k_2}\big(d_1(1-p_2)-d_2(1-p_1)\big)\big(d_1(1-{k_2})-d_2\big)$\\
\hline
$B_2$&$= -p_1^{k_2}(1-p_2)(0.5d_1^2-\beta d_1+\frac{d_1^2}{1-p_1})+(1-p_1)(0.5d_2^2-\beta d_2+\frac{d_2^2}{1-p_2})$\\
	&$  \ \ \  \
	-\big(d_1(1-p_2)-d_2(1-p_1)\big)(d_1-d_2)$\\
\hline
$C_2$&$= (1-p_2)(0.5d_1^2-\beta d_1+\frac{d_1^2}{1-p_1})$ \\
\hline
$D_2$&$= \big(d_2(1-p_1)-d_1(1-p_2)\big)d_1$ \\
\hline\hline
\end{tabular}
\label{notations}
\end{table}

%In Lemma \ref{AVG_COST_THRED}, $J_2(m_2, k_2,\beta)$ and $J_1(m_1, k_1,\beta)$ are calculated with aid of the state transition diagram. 
In Theorem \ref{CONVEXITY}, we provide some nice properties for $J_1$ and $J_2$, which enables us to develop a low-complexity algorithm. To this end, we make a change of variable in Theorem \ref{CONVEXITY} (i), i.e., $m_1$ is replaced with $\log_{p_2}(y)$ in $J_1$, where $y\in (0,1]$.
Some notations used in this theorem are defined in Table \ref{notations}.

%\begin{lemma}
%\label{AVG_COST_THRED} 
%
%(i) The average cost under the policy in \eqref{type1} is 
%	\begin{equation}
%		J_2(m_2, k_2,\beta)=\frac{A_1p_1^{2m_2}+B_1p_1^{m_2}+C_1+D_1m_2p_1^{m_2}}{1-p_2+(1-p_1-p_1^{k_2}(1-p_2))p_1^{m_2}}.
%		\label{cost1}
%	\end{equation}
%%where 
%%\begin{align}
%%	A_1=&p_1^{k_2}\big(d_1(1-p_2)-d_2(1-p_1)\big)\big(d_1(1-{k_2})-d_2\big),\\
%%	B_1=&-\big(d_1(1-p_2)-d_2(1-p_1)\big)(d_1-d_2)\notag\\
%%	&-p_1^{k_2}(1-p_2)(0.5d_1^2-\beta d_1)-\frac{p_1^{k_2}(1-p_2)d_1^2}{1-p_1}\notag\\
%%	&+(1-p_1)(0.5d_2^2-\beta d_2)+\frac{d_2^2(1-p_1)}{1-p_2},\\
%%	C_1=&(1-p_2)(0.5d_1^2-\beta d_1+\frac{d_1^2}{1-p_1}),\\
%%    D_1=&\big(d_2(1-p_1)-d_1(1-p_2)\big)d_1.
%%\end{align}
%
%(ii) The average cost under the policy in \eqref{type2} is 
%\begin{equation}
% 	J_1(m_1, k_1,\beta)=\frac{A_2p_2^{2m_1}+B_2p_2^{m_1}+C_2+D_2m_1p_2^{m_1}}{1-p_1+(-1+p_1+p_2^{k_1}(1-p_2))p_2^{m_2}}.
% 	\label{cost2}
% \end{equation}
%%where
%%\begin{align}
%%	A_2=& p_2^{k_1}\big(d_2(1-p_1)-d_1(1-p_2)\big)\big(d_2(k_1+1)-d_1\big),\\
%%	B_2=& -A_2+\frac{d_1^2p_2^{k_1}(1-p_2)}{1-p_1}-\frac{d_2^2(1-p_1)}{1-p_2}\notag\\
%%	&+p_2^{k_1}(1-p_2)(0.5d_1^2-\beta d_1)+(1-p_1)(\beta d_2-0.5d_2^2),\\
%%	C_2=& (1-p_1)(0.5d_2^2-\beta d_2+\frac{1}{1-p_2})d_2^2,\\
%%	D_2=& \big(d_1(1-p_2)-d_2(1-p_1)\big)d_2p_2^{k_1}.
%%\end{align}
%\end{lemma}
%%\begin{proof}
%%	Please see Appendix \ref{cost_cal}.
%%\end{proof}
%\ifreport
%\begin{proof}
%See Appendix \ref{cost_cal}.
%\end{proof}
%\else 
%\begin{proof}
%See our technical report \cite{yao2020age}.
%\end{proof}
%\fi

%\textbf{Step (ii): Find the $\beta$ associated optimal policy $\pi^*_\beta$: }
\begin{theorem}
\label{CONVEXITY} 
Given $\beta\in [\beta_\text{min}, \beta_\text{max}]$,

(i) if $d_1(1-p_2)<d_2(1-p_1)$, then the average cost is given by 
\begin{equation}
 	J_1(y, k_1,\beta)=\frac{A_1y^{2}+B_1y+C_1+D_1y\log_{p_2}(y)}{1-p_1+(-1+p_1+p_2^{k_1}(1-p_2))y},
 	\label{cost2}
 \end{equation}
where $y\triangleq p_2^{m_1}$. Moreover, $J_1(y, k_1,\beta)$ is quasi-convex in $y$ for $0<y\leq 1$, given $k_1\in\mathcal{K}_1$.

(ii) if $d_1(1-p_2)\geq d_2(1-p_1)$, then optimal average cost is given by
	\begin{equation}
		J_2(0, 0,\beta)=\frac{A_2+B_2+C_2}{1-p_1}.
		\label{cost1}
	\end{equation}
Moreover, the average-optimal policy chooses $u=2$ at every transmission opportunity.
\end{theorem}
\ifreport
\begin{proof}
See Appendix \ref{convex_prop}.
\end{proof}
\else 
\begin{proof}
Proof of part (i) is provided in Appendix \ref{convex_prop}. For part (ii), the key idea is to show that for all $m_2$,
 $J_2(m_2, k_2,\beta)$ is non-decreasing in $k_2\in \mathcal{K}_2$, and then $J_2(m_2, 0,\beta)$ is non-decreasing in $m_2$. This implies that the optimal decision is $u=2$ at each transmission opportunity. Due to the space limitation, detailed proof is provided in our technical report \cite{yao2020age}.
\end{proof}
\fi
 
With the property in Theorem \ref{CONVEXITY} (i), we are able to use golden section search \cite{press2007section} to find the optimal value of $y$ under condition $d_1(1-p_2)<d_2(1-p_1)$. The details are provided in Algorithm \ref{alg1} (Line 12-20).
 Note that $\log_{p_2}(\cdot)$ is one-to-one functions. Thus, after obtaining the optimal $y$ that minimizes $J_1$, the corresponding optimal threshold $m_1$ can be easily obtained by comparing %$J_2(\lfloor\!\log_{p_1}\!(x)\!\rfloor;\! k_2,\!\beta)$ and $J_2(\lceil\! \log_{p_1}\!(x)\!\rceil; \!k_2,\!\beta)$. Similarly, optimal $m_1$ can be obtained by 
$J_1({p_2}^{\lfloor \log_{p_2}(y)\rfloor}, k_1,\beta)$ and $J_1({p_2}^{\lceil \log_{p_2}(y)\rceil}, k_1,\beta)$). The details are provided in Algorithm \ref{alg1} (Line 21-22).
Till now, we have solved $\min_{m_1} J_1(m_1, k_1,\beta)$ given $k_1$ and $\beta$. Note that $k_1\in\mathcal{K}_1$ has finite and countable values. Then, we can easily solve \eqref{target2} under condition $d_1(1-p_2)< d_2(1-p_1)$ by searching for the optimal $k_1$ in the finite set $\mathcal{K}_1$.
%Thus, to solve \eqref{target}, we need to find some nice property of $J_2$ with regard to $m_2$ to solve $\min_{m_2} J_2(m_2, k_2,\beta)$ given $k_2$ and $\beta$. Then, we can easily solve \eqref{target1} by searching for the optimal $k_2$ that minimizes $\min_{m_2} J_2(m_2, k_2,\beta)$. Same method applies to solving \eqref{target2}.
%To get some nice property of $J_2$ with regard to $m_2$ and $J_1$ with regard to $m_1$, we make a change of variable. Specifically, let $x$ be a real-valued variable such that $0<x\leq 1$. We replace $m_2$ with $\log_{p_1}(x)$ in \eqref{cost1} and obtain $J_2(\log_{p_1}(x), k_2,\beta)$ and replace $m_1$ with $\log_{p_2}(x)$ in \eqref{cost2} and obtain $J_1(\log_{p_2}(x), k_1,\beta)$. 
%
%In Theorem \ref{CONVEXITY}, we prove that given $\beta\in [\beta_\text{min}, \beta_\text{max}]$, $k_2\in \mathcal{K}_2$ and $k_1 \in\mathcal{K}_1$, $J_2(\log_{p_1}(x), k_2,\beta)$ is convex in $x$ if $d_1(1-p_2)\geq d_2(1-p_1)$ and $J_1(\log_{p_2}(x), k_1,\beta)$ is quasi-convex in $x$ if $d_1(1-p_2)<d_2(1-p_1)$, where the definitions of quasi-convex is given in Definition \ref{quasi_convex}.  
%\begin{definition}\cite{boyd2004convex}
%\label{quasi_convex}
%	A continuous function $f:\mathbb{R}\rightarrow\mathbb{R}$ is quasiconvex if and only if at least one of the following conditions holds:
%	\begin{itemize}
%		\item $f$ is nondecreasing
%		\item $f$ is nonincreasing
%		\item there is a point $c\in \mathbf{dom} f$ such that for $t\leq c$ (and $t\in \mathbf{dom} f$), $f$ is nonincreasing, and for $t\geq c$ (and $t\in \mathbf{dom} f$), $f$ is nondecreasing.
%	\end{itemize}
%\end{definition}

Note that Theorem \ref{CONVEXITY} (ii) applies to all $\beta\in \![\beta_\text{min},\! \beta_\text{max}\!]$ including $\beta^*$. Thus, the optimal policy for \eqref{equiv1} is to take $u=2$ at every transmission opportunity, which is returned directly in Algorithm \ref{alg1} (Line 4-5). Under this condition, the step (ii) is only used to find optimal average cost $\beta^*$ for \eqref{equiv1}. 

Moreover, in Line 9-10, we add a judgement sentence, i.e., if the condition $\frac{\partial J_1(y,k_1,\beta)}{\partial y}\vert_{y=1}<0$ is satisfied, then we can directly obtain the optimal $m_1$ without running golden section method. This further reduces the algorithm complexity. The judgement is based on the fact that $\lim_{y\rightarrow 0}\frac{\partial J_1(y, k_1,\beta)}{\partial y}<0$ (this is proved in the proof of Theorem \ref{CONVEXITY} in Appendix \ref{convex_prop}) and $J_1$ is quasi-convex. Thus, if $\frac{\partial J_1(y, k_1,\beta)}{\partial y}\vert_{y=1}<0$, then $J_1$ is non-increasing in $y$.

\textbf{Step (ii): Find $\beta^*$:} By Lemma \ref{TRANS}, if $p(\beta)>0$, then $\beta<\beta^*$; if $p(\beta)<0$, then $\beta>\beta^*$. Thus, we can use bisection method to search for $\beta^*$. The details are provided in Algorithm \ref{alg1} (Line 2-3 and Line 29-33). 



